On the Privacy Risks of Algorithmic Fairness

Algorithmic fairness and privacy are essential pillars of trustworthy machine learning. Fair machine learning aims at minimizing discrimination against protected groups by, for example, imposing a constraint on models to equalize their behavior across different groups. This can subsequently change the influence of training data points on the fair model, in a disproportionate way. We study how this can change the information leakage of the model about its training data. We analyze the privacy risks of group fairness (e.g., equalized odds) through the lens of membership inference attacks: inferring whether a data point is used for training a model. We show that fairness comes at the cost of privacy, and this cost is not distributed equally: the information leakage of fair models increases significantly on the unprivileged subgroups, which are the ones for whom we need fair learning. We show that the more biased the training data is, the higher the privacy cost of achieving fairness for the unprivileged subgroups will be. We provide comprehensive empirical analysis for general machine learning algorithms.

==> data/tab-NN-results.tex <==
% !TEX root = ../main.tex

{\renewcommand{\arraystretch}{1.15}
\begin{table}
\caption{\small Privacy risk of unconstrained and fair neural network models (with~$\delta = 0.001$) across different subgroups.}
\label{tab:NN-privacy-cost}
\begin{tabularx}{\columnwidth}{
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
}
\toprule
Dataset & Model & $G_{0}^-$ & $G_{1}^-$ & $G_{0}^+$ &$G_{1}^+$  \\ \hline
Bank&Unconstrained&${0.523}^*$&0.505&0.548&${0.513}^*$\\
(age)&Fair&0.523&0.504&0.548&0.513\\
\hline\hline
COMPAS&Unconstrained&${0.579}^*$&0.568&0.573&${0.608}^*$\\
(race)&Fair&0.586&0.578&0.582&0.625\\
\hline\hline
COMPAS&Unconstrained&0.578&${0.575}^*$&0.632&${0.568}^*$\\
(gender)&Fair&0.575&0.586&0.641&0.582\\
\hline\hline
Law&Unconstrained&0.610&${0.589}^*$&0.524&0.507\\
(race)&Fair&0.604&0.628&0.525&0.507\\
\hline\hline
Law&Unconstrained&0.613&${0.600}^*$&0.511&0.509\\
(gender)&Fair&0.631&0.642&0.512&0.511\\
\toprule
\end{tabularx}
\end{table}
}









==> data/tab-classification-performance-paper.tex <==
% !TEX root = ../main.tex


{\renewcommand{\arraystretch}{1.15}
\begin{table}[t!]
\caption{ Accuracy and fairness gap of unconstrained models and fair models on the training dataset and the test dataset. The ``Train $\Delta$'' and ``Test $\Delta$'' columns show the results for the fairness gap on the training data and the test data which is defined in ~\eqref{eq:eo-fairness}.}
\begin{tabularx}{\columnwidth}{
 c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
}
\toprule
Model & Train acc& Test acc & Train $\Delta$ & Test $\Delta$ \\ \hline
Unconstrained& 86.2\%& 85.5\%& 0.373&0.430\\
% Fair ($\delta=0.1$)& 89.1\%&87.8\%&0.105&0.332\\
% Fair ($\delta=0.01$)&85.6\% &84.0\%&0.014 &0.283\\
Fair ($\delta=0.001$)&84.5\%&83.8\%&0.001&0.275\\
\bottomrule
\label{tab:accuracy_synthetic_paper}
\end{tabularx}
\end{table}
}


==> data/tab-classification-performance-real-data-paper.tex <==

% !TEX root = ../main.tex

{\renewcommand{\arraystretch}{1.15}
\begin{table}[t!]
\caption{Accuracy and fairness gap of unconstrained models and fair models ($\delta=0.001$) on the training dataset and test dataset -- Decision tree model with max depth 10.}
\label{tab:prediction_acc_real_paper}
\begin{tabularx}{\columnwidth}{
% c
%  c
c
c
 >{\centering\arraybackslash}X c
 >{\centering\arraybackslash}X c
 >{\centering\arraybackslash}X c
 >{\centering\arraybackslash}X c
 }
 \toprule
 Dataset & Model & Train acc & Test acc & Train $\Delta$ & Test $\Delta$  \\ \hline
Bank&
Unconstrained&92.5\%&87.8\%&0.063&0.074\\
&Fair ($\delta=0.001$)&94.6\%&89.3\%&0.001&0.066\\


 \hline\hline
COMPAS&
Unconstrained&72.4\%&60.1\%&0.097&0.133\\
% &Fair ($\delta=0.1$)& 79.4\%&64.3\%&0.108&0.131\\
% \multirow{1}{*}{(race)}&Fair ($\delta=0.01$)& 79\%&64\%&0.017&0.073\\
(race)&Fair ($\delta=0.001$)&78.7\%&64\%&0.002&0.067\\


 \hline\hline

COMPAS&
Unconstrained&72.4\%&60.2\%&0.117&0.107\\
% &Fair ($\delta=0.1$)&79.3\%&64.4\%&0.081&0.1 \\
% \multirow{1}{*}{(gender)}&Fair ($\delta=0.01$)& 78.6\%&64.4\%&0.013&0.083\\
(gender)&Fair ($\delta=0.001$)&78.5\%&64.3\%&0.001&0.08\\

 \hline\hline
Law&
Unconstrained&95.9\%&92.2\%&0.236&0.165\\
% &Fair ($\delta=0.1$)& 97.6\%&93.6\%&0.148&0.156\\
% \multirow{1}{*}{(race)}&Fair ($\delta=0.01$)&97.5\%&93.4\%&0.018&0.12 \\
(race)&Fair ($\delta=0.001$)&97.5\%&93.5\%&0.002&0.112\\

 \hline\hline
Law&
Unconstrained&95.9\%&92.2\%&0.035&0.039\\
% &Fair ($\delta=0.1$)& 97.6\%&93.6\%&0.097&0.039\\
% \multirow{1}{*}{(gender)}&Fair ($\delta=0.01$)& 97.6\%&93.6\%&0.019&0.04\\
(gender)&Fair ($\delta=0.001$)&97.6\%&93.6\%&0.002&0.033\\
 \bottomrule
 \end{tabularx}
 \label{tab:accuracy_real_data}
 \end{table}
 }


==> data/tab-different-delat-paper.tex <==
% !TEX root = ../main.tex



% different delta

{\renewcommand{\arraystretch}{1.15}
\begin{table}[t!]
\caption{ Privacy risk of unconstrained models and fair models with different enforced fairness gap $\delta$ on decision tree models with max depth 10 -- Law (race) dataset.}
\begin{tabularx}{\columnwidth}{
c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
>{\centering\arraybackslash}X c
}
\toprule
Model & $G_{0}^-$& $G_{1}^-$ & $G_{0}^+$ &$G_{1}^+$  \\ \hline
 Unconstrained&72.6\%&71.1\%&54.1\%&51.0\%\\
Fair ($\delta=0.1$)&74.4\%&77.7\%&55.0\%&51.3\%\\
Fair ($\delta=0.01$)&74.3\%&81.0\%&55.3\%&51.4\%\\
Fair ($\delta=0.001$)&74.5\%&81.8\%&55.5\%&51.5\%\\
\bottomrule
\end{tabularx}
\label{tab:different_delta_paper}
\end{table}
}


==> data/tab-notations.tex <==
% !TEX root = ../main.tex

\begin{table}[h]
	\centering
	\caption{\small Table of notation}
\begin{tabular}{p{0.1\columnwidth}p{0.8\columnwidth}p{0.1\columnwidth}}
	\hline
	\textbf{Symbol} & \textbf{Description} & \textbf{Section}\\ \hline
	  $\M$ & Machine learning model. & \ref{subsec:machine_learning}\\
	  $\X$ & Feature space. & \ref{subsec:machine_learning}\\
	  $\Y$ & Label space & \ref{subsec:machine_learning}\\
	  $\ell$ & Loss function. & \ref{subsec:machine_learning} \\
      $\train$ & Training set.  & \ref{subsec:machine_learning}\\
      $n$ & Size of the training set.  & \ref{subsec:machine_learning}\\
      $\M_\train$ & Machine learning model trained on $\train$. & \ref{subsec:machine_learning}\\ 
      $\D$ & Data distribution. & \ref{subsec:machine_learning}\\
      $z$ & Data point. & \ref{subsec:fairness}\\
      $x$ & Feature vector. & \ref{subsec:machine_learning}\\
      $g$ & Protected attribute. & \ref{subsec:machine_learning}\\
      $y$ & Label. & \ref{subsec:machine_learning}\\
      $\G$ & Protected attribute space. & \ref{subsec:machine_learning}\\
      $\D_{g}^y$ & Distribution of the data with protected attribute $g$ and label $y$. & \ref{subsec:fairness}\\
      $X$ & Random variable associated with feature vector. & \ref{subsec:machine_learning}\\
      $Y$ & Random variable associated with label. & \ref{subsec:machine_learning}\\
      $G$ & Random variable associated with protected attribute. & \ref{subsec:machine_learning}\\
      $G_{g}$ & A set of points in dataset $\train$ with protected attribute g. & \ref{subsec:fairness}\\
      $G_{g}^y$ & A set of points in dataset $\train$ with protected attribute g and label y. & \ref{subsec:fairness}\\
      $\Delta$ & Fairness gap. & \ref{subsec:fairness}\\
      $\delta$ & Enforced fairness level. & \ref{subsec:fairness}\\
      $b$ & The secret bit chosen by the challenger. & \ref{subsec:privacy_risk}\\
      $A$ & An algorithm. &  \ref{subsec:privacy_risk}\\
      $A_\train$ & The output of algorithm $\A$ on dataset $\train$.&  \ref{subsec:privacy_risk}\\
      $\hat{b}$ & Adversary's guess of $b$. & \ref{subsec:privacy_risk}\\
      $\mathcal{A}$ & Membership inference attack. & \ref{subsec:privacy_risk}\\
      $\tau^{(g,y)}$ &  The loss threshold used by the adversary for subgroup $G_g^y$. &  \ref{subsec:privacy_risk}\\
      $\mathcal{N}$ & Gaussian distribution. &  \ref{sec:evaluation}\\
	\hline
\end{tabular}
\label{table:notations}
\end{table}





==> figure_scripts/toy_example.tex <==
% !TEX root = ../main.tex
\begin{figure*}[t!]
	\centering
	\if\compileFigures1
  \resizebox{\textwidth}{!}{\input{figure_scripts/fig_toy_example_change_n0}}
    \resizebox{\textwidth}{!}{\input{figure_scripts/fig_toy_example_change_point}}
	\else
	\resizebox{\textwidth}{!}{\includegraphics[]{fig/\filename-figure\thefigureNumber.pdf}}
	\stepcounter{figureNumber}
	\resizebox{\textwidth}{!}{\includegraphics[]{fig/\filename-figure\thefigureNumber.pdf}}
	\stepcounter{figureNumber}
	\fi
	\caption{Individual privacy risk, following the theoretical analysis in Section~\ref{subsec:toy-example}. For all settings, we set ${\mu_0 = 0}$, ${\mu_1=2}, {\sigma_0 = 1}$ and ${\sigma_1 =2}$.
		The x-axis is the true positive rate of the attack, and the y-axis is the true negative rate. We vary the value of $n_0$ while keeping $n_1 = 400$  for measuring the privacy risk for ${-3,0}$ (shown in the first row). In the second row, we fix the $n_0, n_1$ and measure the individual privacy risk for different points. For each model, the privacy risk of the challenge point $z$ (i.e., the maximum of $1-\frac{\alpha + \beta}{2}$) is reported in each plot. The numbers with blue color represent the privacy risks in the standard setting, and the numbers with red color represent privacy risks in the fair setting.}
	\label{fig:toy-example-change-size}
\end{figure*}


==> figure_scripts/toy_example_new.tex <==
% !TEX root = ../main.tex
\begin{figure*}[t!]
	\centering
	\if\compileFigures1
  \resizebox{\textwidth}{!}{\input{figure_scripts/fig_toy_example_change_n0_new}}
    \resizebox{\textwidth}{!}{\input{figure_scripts/fig_toy_example_change_point_new}}
	\else
	\resizebox{\textwidth}{!}{\includegraphics[]{fig/\filename-figure\thefigureNumber.pdf}}
	\stepcounter{figureNumber}
	\resizebox{\textwidth}{!}{\includegraphics[]{fig/\filename-figure\thefigureNumber.pdf}}
	\stepcounter{figureNumber}
	\fi
	\caption{Individual privacy risk, following the theoretical analysis in Section~\ref{subsec:toy-example}. For all settings, we set ${\mu_0 = 0}$, ${\mu_1=2}, {\sigma_0 = 1}$ and ${\sigma_1 =2}$.
		The x-axis is the false positive rate of the attack (i.e., $\alpha$), and the y-axis is the true positive rate (i.e., $1-\beta$). We vary the value of $n_0$ while keeping $n_1 = 400$  for measuring the privacy risk for ${(-4,0)}$ (shown in the first row). In the second row, we fix the $n_0, n_1$ and measure the individual privacy risk for different points. For each model, the privacy risk of the challenge point $z$ (i.e., the maximum of $1-\frac{\alpha + \beta}{2}$) is reported in each plot. The numbers with blue color represent the privacy risks in the standard setting, and the numbers with red color represent privacy risks in the fair setting.}
	\label{fig:toy-example-change-size}
\end{figure*}


==> sections/sec_discussion.tex <==
% !TEX root = ../main.tex

\section{Discussion About Countermeasures}\label{sec:discussion}

A rigorous framework to protect privacy is to use differentially private training algorithms to bound information leakage about members of the training data. 
More precisely, for a given false positive rate, the true positive rate of the membership inference attacks is upper bounded in differentially private models (as shown in Proposition-1 \cite{erlingsson2019we}). Thus, the privacy risk (in Definition 2) is upper bounded by $\frac{(e^\epsilon-1)+\delta+1}{2}$ when the model is $(\epsilon,\delta)$-differentially private (for all the individuals regardless of their subgroups).


It is worth highlighting that, \citet{jagielski2019differentially} shows that, for two algorithms proposed in their paper, the algorithms achieve fairness and differential privacy at the same time. Thus, those algorithm achieves fairness while preserving privacy. 
The major observation, however, is that model accuracy significantly drops. 
%
At the same time, in our paper, we show that when the accuracy on the unprivileged subgroup increases after imposing fairness constraints, the corresponding privacy risk will be increased. On the other hand, if the accuracy does not increase after imposing fairness constraints (e.g., fair models trained using post-processing algorithm), there might not be a privacy cost of fairness as the accuracy cost of fairness is already large.

Based on these, we suspect that there might be an inherent trade-off between privacy, fairness, and accuracy. Investigating this trade-off from theoretical perspectives would be a promising future research direction.



==> sections/subsec_framework-a-toy-example.tex <==
% !TEX root = ../main.tex

\section{Theoretical Privacy Analysis of Fair Mean}\label{subsec:toy-example}
We consider the problem of releasing the empirical mean of a dataset $S$ with a single attribute $X$ in $\mathbb{R}$, where the records belong to individuals from two groups (e.g., distinguished by their race).  We assume the data points in group $g$ are distributed according to probability distribution $\D_g$ with mean $\mu_g$.  

\begin{definition}[Fair Mean]
	We define $\mu$ to be a fair mean, across two groups $g \in \{0, 1\}$, if ${|\mu - \mu_0| = |\mu - \mu_1|}.$
\end{definition}

This is similar to the fairness definition in the prior work which defines fairness as equality of loss across two groups~\cite{khani2020feature, donini2018empirical}.  Consider the loss of a data point in group $g$ as its squared distance to the released mean. If the variances of $\D_0$ and $\D_1$ are the same, this fairness definition implies that the expected loss for two groups should be the same: 
%
\begin{align*}
	\mathbb{E}_{X \sim \D_0}\Big[(X - \mu)^2\Big] =\mathbb{E}_{X \sim \D_1}\Big[(X - \mu)^2\Big] .
\end{align*}

According to the definition of fair mean, we compute the empirical fair mean of $S$ as $\hat{\mu}^{\mathrm{f}} = {\frac{1}{2} (\hat{\mu}_0+ \hat{\mu}_1)}$, where $\hat{\mu}_g$ is the empirical mean of $S$ for elements in group $g$.



\subsubsection*{Privacy Risk Analysis}

We assume the adversary knows the number of data points in each group (i.e., $n_0$, $n_1$), and aims to infer whether a given data point $z$ (whose group membership is known to both adversary and challenger) is part of $S$, by observing the released mean (which is empirical mean~$\hat{\mu}$ in the standard setting, and~$\hat{\mu}^{\mathrm{f}}$ in the fair setting).

We analyze membership inference attacks, by modeling the attacks as a likelihood ratio test~\cite{sankararaman2009genomic, murakonda2021quantifying}.\footnote{According to the Neyman-Pearson lemma~\cite{neyman1933ix}, the likelihood ratio test achieves the maximum power (true positive rate) among all tests, for any given error (false positive rate).  In other words, for any given false positive rate, there exists no other attack strategy that can achieve a higher true positive rate.}  The adversary's objective is to distinguish between two hypotheses, which describe the possible world that could have resulted in the adversary's observation. In one world (alternative hypothesis), the data point $z$ is a member of set $S$, and in the other one (null hypothesis), the data point is not part of $S$.
%
\begin{align*}
	& \mathrm{H}_0: z \notin S \quad \mbox{Null hypothesis (non-member)}\\
	& \mathrm{H}_1: z \in S \quad \mbox{Alternative hypothesis (member)}
\end{align*}

Attacker compares the likelihood of the released mean under these two hypotheses.  The log likelihood ratio of the released $\mu$ is computed as follows:
%
\begin{align*}
	L(z) = \log\left(\frac{\Pr[z ; \mu, \mathrm{H}_0 \mbox{ is true}]}{ \Pr[ z ; \mu, \mathrm{H}_1 \mbox{ is true}]}\right).
\end{align*}

The likelihood ratio test is a comparison of $L(z)$ with a threshold $\tau$.  If $L(z) \leq \tau$, then the attacker rejects the null hypothesis and decides in favor of $\mathcal{H}_1$ (i.e., predicts $z \in S$); otherwise, he predicts $z \notin S$, as there is not enough evidence to reject the null hypothesis.

In the next, we assume $X$ follows the Gaussian distribution $\mathcal{N}(\mu_g,\sigma_g^2)$, for $g \in \{0, 1\}$ and assume that there are $n_g$ data points of $S$ with $G=g$.



\subsubsection*{Standard setting}
In this setting, the adversary only observes the mean of $S$ defined as $\hat{\mu} \triangleq \frac{1}{n} \sum_{i=1}^n X_i$. Accordingly, the empirical mean follows a Gaussian distribution. 
More precisely, 
\begin{align*}
&\mbox{when }  \mathrm{H}_0 \mbox{ is true, } \hat{\mu} \sim \mathcal{N}(\bar{\mu},\bar{\sigma}^2) , \mbox{ and } \\
&\mbox{when }  \mathrm{H}_1 \mbox{ is true,  } \hat{\mu}\sim \mathcal{N}(\bar{\mu}+\frac{x-\mu_g}{n}, \bar{\sigma}^2 - \frac{\sigma_g^2}{n^2}) ,
\end{align*}
%
where $\bar{\mu} = \frac{n_0 \mu_0+ n_1 \mu_1}{(n_0 + n_1)}$, $\bar{\sigma}= \sqrt{\frac{n_0\sigma_0^2 + n_1 \sigma_1^2}{(n_0 + n_1)^2}}$, and ${x, g}$ are the attribute and group of $z$ respectively.

We find that the difference in the variance is small (i.e., $\frac{\sigma_g^2}{n^2}$). When $n^2 \gg \sigma_g^2$, the difference in the variance approaches to 0. When it is 0, the threshold $\tau$ for the log-likelihood ratio test can be converted to the threshold for the $\hat{\mu}$. In other words, the adversary only needs to find a threshold $\tau$ and compare the $\hat{\mu}$ with the threshold $\tau$.
Thus, we estimate the likelihood ratio test by comparing a threshold with the empirical mean $\hat{\mu}$.
Let $\alpha$ be the false positive rate and $\beta$ be the false negative rate of the attacker. We obtain the relation between $\alpha$ and $\beta$ as follows:
%
\begin{align}\label{eq:power_of_attack_un}
   F^{-1}(1-\beta) \sqrt{\bar{\sigma}^2 - \frac{\bar{\sigma}_g^2}{n^2}} -  \bar{\sigma} F^{-1}(\alpha)   = \Big|\frac{x-\mu_g}{n}\Big|,
\end{align}
%
where $F^{-1}$ is the inverse CDF of a standard normal distribution. This shows that, given a fixed false positive rate $\alpha$, the false negative rate $\beta$ of any attack (hypothesis test) is lower bounded.


\subsubsection*{Fair setting} 


Thus, in this fair setting, adversary observes $\hat{\mu}^{\mathrm{f}} $. The likelihood of the fair mean also follows the Gaussian distribution:
\begin{align*}
	&\mbox{when }  \mathrm{H}_0 \mbox{ is true,  } \hat{\mu}^{\mathrm{f}}  \sim \mathcal{N}(\bar{\mu}_f,\bar{\sigma}_f^2) , \mbox{ and } \\
	&\mbox{when }  \mathrm{H}_1 \mbox{ is true,  } \hat{\mu}^{\mathrm{f}}  \sim \mathcal{N}(\bar{\mu}_f+\frac{x-\mu_g}{2n_g}, \bar{\sigma}_f^2 - \frac{\sigma_g^2}{4n_g^2}) ,
\end{align*}
where $\bar{\mu}_f = \frac{\mu_0+\mu_1}{2}$ and $\bar{\sigma}_f= \sqrt{\frac{\sigma_0^2/n_0 +\sigma_1^2/n_1}{4}}$.
Similarly, we obtain the relation between $\alpha$ and $\beta$ as follows:
\begin{align}\label{eq:power_of_attack_fair}
   F^{-1}(1-\beta) \sqrt{\bar{\sigma}_f^2 - \frac{\sigma_g^2}{4n_g^2}}  - \bar{\sigma}_f F^{-1}(\alpha)  = \Big|\frac{x-\mu_g}{2n_g}\Big|
\end{align}
Next, we show the numerical computation of the privacy risk in different settings.
\subsubsection*{Numerical Computation}
Figure~\ref{fig:toy-example-change-size}  shows the privacy risk of the challenge point in the standard setting and fair setting.
 \input{figure_scripts/toy_example}

We observe that, when $n_0$ is much smaller than $n_1$, with a fixed true positive rate, the attacker can achieve a much better true negative rate in the fair setting, which means that \emph{the information leakage of the fair empirical mean about the challenge point is much more than that of the empirical mean}.
In addition, we also report the privacy risk, which is the maximum attack accuracy (i.e., $1- (\alpha+\beta)/2$) over all possible attacks.
As $n_0$ decreases, the attack accuracy increases significantly in the fair setting. On the other hand, the accuracy is barely changed in the standard setting.

Besides, when $n_0=10$, the subgroup privacy risk in the standard setting is 50.4\% for both group $G_0$ and group $G_1$.
 On the contrary, in the fair setting, the subgroup privacy risk is 50.1\% for group $G_0$ and 55.3\% for group $G_1$. It shows that the changes in the privacy risk caused by the fairness requirement are different for each group.
This is in agreement with our empirical results.


==> sections/subsec_framework-a-toy-example_new.tex <==
% !TEX root = ../main.tex

\subsection{Theoretical Privacy Analysis of Fair Mean}\label{subsec:toy-example}

We consider the problem of releasing the empirical mean of a dataset $S$ of size $n$ with a single attribute $X$ in $\mathbb{R}$, where the records belong to individuals from two groups (e.g., distinguished by their race).  We assume the data points in group $G_g$ are distributed according to probability distribution $\D_g$ with mean $\mu_g$ and $S$ contains $n_g$ data points from group $G_g$.

\begin{definition}[Fair Mean]
	We define $\mu$ to be a fair mean, across two groups $g \in \{0, 1\}$, if ${|\mu - \mu_0| = |\mu - \mu_1|}.$
\end{definition}

This is similar to the fairness definition in the prior work, which defines fairness as equality of loss across two groups~\cite{khani2020feature, donini2018empirical}.  Consider the loss of a data point in the group $G_g$ as its squared distance to the released mean. If the variances of $\D_0$ and $\D_1$ are the same, this fairness definition implies that the expected loss for two groups should be the same: 
%
\begin{align*}
	\mathbb{E}_{X \sim \D_0}\Big[(X - \mu)^2\Big] =\mathbb{E}_{X \sim \D_1}\Big[(X - \mu)^2\Big] .
\end{align*}

According to the definition of fair mean, we compute the empirical fair mean of $S$ as ${O^{\mathrm{f}}  = \frac{1}{2} (\bar{X}_0+ \bar{X}_1)}$, where $\bar{X}_g$ is the empirical mean of $S$ for elements in group $G_g$.
%$\hat{\mu}^{\mathrm{f}} = {\frac{1}{2} (\hat{\mu}_0+ \hat{\mu}_1)}$ not necessary.

\subsubsection*{Privacy Risk Analysis}

We assume the adversary knows the number of data points in each group (i.e., $n_0$, $n_1$) and the data distribution for each group. He aims to infer whether a given data point $z$ (which is known to the adversary) is part of $S$, by observing the released mean $O$ (which is empirical mean~$O^{\mathrm{u}}$ in the standard setting, and empirical fair mean~${O^{\mathrm{f}}}$ in the fair setting).

We analyze membership inference attacks by modeling the attacks as a likelihood ratio test~\cite{sankararaman2009genomic, murakonda2021quantifying}.\footnote{According to the Neyman-Pearson lemma~\cite{neyman1933ix}, the likelihood ratio test achieves the maximum power (true positive rate) among all tests, for any given error (false positive rate).  In other words, for any given false positive rate, there exists no other attack strategy that can achieve a higher true positive rate.}  The adversary's objective is to distinguish between two hypotheses, which describe the possible world that could have resulted in the adversary's observation. In one world (alternative hypothesis), the data point $z$ is a member of set $S$. In this case, ${S = S' \cup \{z\}}$, where ${ S' \sim \D^{n-1}}$. In the other one (null hypothesis), the data point is not part of $S$, thus ${S \sim \D^n}$. We let ${Q^{1,z}}$ and ${Q^{0}}$ denote the distribution of released mean $O$ in those two cases, respectively. 
%
\begin{align*}
	& \mathrm{H}_0: O \sim Q^0   \quad \enspace \mbox{Null hypothesis } (z \notin S)\\
	& \mathrm{H}_1:  O \sim Q^{1,z} \quad \mbox{Alternative hypothesis }(z \notin S)
\end{align*}

Attacker compares the likelihood of the released mean under these two hypotheses.  The log-likelihood ratio of the released mean $o$ for a given $z$ is computed as follows:
%
\begin{align*}
	L(o, z) = \log\left(\frac{\Pr[o ; z, \mathrm{H}_0 \mbox{ is true}]}{ \Pr[ o ; z, \mathrm{H}_1 \mbox{ is true}]}\right) =  \log\left(\frac{\Pr_{Q^0}[O=o]}{ \Pr_{Q^{1,z}}[O=o]}\right).
\end{align*}

The likelihood ratio test is a comparison of $L(o, z)$ with a threshold $\tau$. On a given $z$, if $L(o, z) \leq \tau$, then the attacker rejects the null hypothesis and decides in favor of $\mathrm{H}_1$ (i.e., predicts $z \in S$); otherwise, he predicts $z \notin S$, as there is not enough evidence to reject the null hypothesis.
For a given error (false positive rate) $\alpha$ that the adversary is willing to tolerate, he can compute the threshold that maximizes his power (true positive rate ${1-\beta}$).

Next, we find the relation between $\alpha$ and $\beta$ which enables us to compute the privacy risk theoretically, under the assumption that $X$  in group $G_g$ follows the Gaussian distribution $\mathcal{N}(\mu_g,\sigma_g^2)$, for $g \in \{0, 1\}$.  

\subsubsection*{Standard setting}
In this setting, the adversary only observes the empirical mean of $S$. Accordingly, on the given $z$,  the distribution of the ${O^\mathrm{u}}$ under different hypotheses, on the given $z = (x, g)$, are shown below:
%
\begin{align*}
	& \mathrm{H}_0: O^\mathrm{u} = \frac{1}{n} \sum_{X \in S} X,  \mbox{thus } Q^0 = \mathcal{N}(\bar{\mu},\bar{\sigma}^2), \\
	& \mathrm{H}_1: O^\mathrm{u} = \frac{1}{n} \sum_{X \in S'} X + x, \mbox{thus }  Q^{1,z} = \mathcal{N}(\bar{\mu'}, \bar{\sigma'}^2),
\end{align*}
where $a\in \{0,1\},  \bar{\mu} = \frac{n_0 \mu_0+ n_1 \mu_1}{(n_0 + n_1)}$, $\bar{\sigma}= \sqrt{\frac{n_0\sigma_0^2 + n_1 \sigma_1^2}{(n_0 + n_1)^2}}$,  $\bar{\mu'} = \bar{\mu}+\frac{x-\mu_g}{n}$, $\bar{\sigma'}^2 =\bar{\sigma}^2 - \frac{\sigma_g^2}{n^2}$. It is clear that, $\bar{\sigma'} < \bar{\sigma}$. In this case, the log-likelihood can be written as follows:
%
\begin{align*}
	L(o,z) &= \log\left(\frac{\Pr[o; z, \mathrm{H}_0 \mbox{ is true} ]}{ \Pr[ o; z, \mathrm{H}_1 \mbox{ is true}]}\right) \\
	&= \log \frac{\esigmad}{\esigmau} - \frac{\big(\emud - \emuu\big)^2}{\sqrt{\esigmau^2 - \esigmad^2}} \\
	& \quad + \frac{1}{2 \esigmad^2} \left(  \frac{\sqrt{\esigmau^2 - \esigmad^2} (o - \emuu)}{\esigmau} - \frac{\esigmau (\emud - \emuu)}{\sqrt{\esigmau^2 - \esigmad^2}} \right)^2. \\ 
\end{align*}

Based on this reformulation, the likelihood ratio test (i.e.,  $L(o,z) > \tau$) can be written as follows:
%
\begin{align*}
	&\left( \frac{\sqrt{\esigmau^2 - \esigmad^2}  (o- \emuu)}{\esigmau} - \frac{\esigmau (\emud - \emuu)}{\sqrt{\esigmau^2 - \esigmad^2}} \right)^2   \\
	& \qquad \quad > 2 \esigmad^2 \left ( \tau  - \frac{\big(\emud - \emuu\big)^2}{\sqrt{\esigmau^2 - \esigmad^2}} - \log \frac{\esigmad}{\esigmau}  \right).
\end{align*}

If the right-hand side is negative, the strategy is to always accept the Null hypothesis because $L(o,z)$ is always greater than any $\tau$.  Next, we consider the case when the right-hand side is non-negative. By introducing a non-negative threshold $\tilde{\tau}$ and simple reformulation, the likelihood ratio test (${L(o,z) > \tau}$) can be equivalently expressed as follows:
% 
\begin{align}\label{eq:region}
	& o \in \mathcal{O}, \nonumber \\
	\mathcal{O} = \{o| o > \frac{\esigmau^2 \emud - \esigmad^2 \emuu}{{\esigmau^2 - \esigmad^2}} &+ \tilde{\tau} \mbox{ or } o < \frac{\esigmau^2 \emud - \esigmad^2 \emuu}{{\esigmau^2 - \esigmad^2}} - \tilde{\tau}\}.
\end{align}

Thus, in this case, the membership inference attack is essentially finding a non-negative threshold $\tilde{\tau}$. The adversary predicts $z$ as ``non-member'' if the empirical mean lies in the region $\mathcal{O}$ defined in \eqref{eq:region} and as ``member'' when empirical mean lies in the complement of $\mathcal{O}$, denoted as $\mathcal{O}^c$. Recall that $\alpha$ is the false positive rate, and $\beta$ is the false negative rate of the likelihood ratio test.  On a non-negative $\tilde{\tau}$, we can compute the $\alpha$ and $1-\beta$.
%
\begin{align}\label{eq:relation-alpha}
	\alpha  &= \int_{o \in \mathcal{O}^c} \Pr_{Q^0}[O=o]do \nonumber \\
	&=F( \frac{\esigmau \big( \emud - \emuu\big)}{\esigmau^2 - \esigmad^2}+ \tilde{\tau} ) - F( \frac{\esigmau \big( \emud - \emuu\big)}{\esigmau^2 - \esigmad^2} - \tilde{\tau})  \nonumber \nonumber \\
\end{align}
where $F$ is the CDF of a standard normal distribution.
Similarly, we can compute $1-\beta$ as follows:
\begin{align}\label{eq:relation-beta}
	1 - \beta &=   \int_{o \in \mathcal{O}^c} \Pr_{Q^{1,z}}[O=o]do \nonumber \\
	&=F( \frac{\esigmad (\emud - \emuu)}{\esigmau^2 (\esigmau^2 - \esigmad^2)} + \frac{\esigmau}{\esigmad}  \tilde{\tau}) - F( \frac{\esigmad (\emud - \emuu)}{\esigmau^2 (\esigmau^2 - \esigmad^2)} - \frac{\esigmau}{\esigmad}  \tilde{\tau})  
\end{align}

This implies that, given a fixed false positive rate $\alpha$, the true positive rate $1-\beta$ of any attack (hypothesis test) is upper bounded. 


\subsubsection*{Fair setting} 
In this fair setting, adversary observes $O^\mathrm{f}$. The fair mean also follows the Gaussian distribution:
%
\begin{align*}
	& \mathrm{H}_0: Q^0 =  \mathcal{N}(\bar{\mu}^\mathrm{f},(\bar{\sigma}^\mathrm{f})^2)  \\
	& \mathrm{H}_1: Q^{1,z} = \mathcal{N}(\bar{\mu'}^\mathrm{f}, (\bar{\sigma'}^\mathrm{f})^2) 
\end{align*}
where $ \bar{\mu}^\mathrm{f} = \frac{\mu_0+\mu_1}{2}$, ${\bar{\sigma}^\mathrm{f}=  \sqrt{\frac{\sigma_0^2/n_0 +\sigma_1^2/n_1}{4}}}$, ${\bar{\mu'}^\mathrm{f} = \bar{\mu}^\mathrm{f}+\frac{x-\mu_g}{2n_g}}$, and ${ (\bar{\sigma'}^\mathrm{f})^2 = (\bar{\sigma}^\mathrm{f})^2 - \frac{\sigma_g^2}{4n_g^2}}$. Similarly, we obtain the relation between $\alpha$ and $\beta$ as shown in~\eqref{eq:relation-alpha} and \eqref{eq:relation-beta}, by replacing the $\emuu, \emud, \esigmau, \esigmad$ with $\emuu^\mathrm{f}, \emud^\mathrm{f}, \esigmau^\mathrm{f}, \esigmad^\mathrm{f}$.
Next, we show the numerical computation of the privacy risk in different settings.


\input{figure_scripts/toy_example_new}
\subsubsection*{Numerical Computation}

Figure~\ref{fig:toy-example-change-size}  shows the privacy risk of the challenge point in the standard setting and fair setting.

We observe that, when $n_0$ is much smaller than $n_1$, with a fixed true positive rate, the attacker can achieve a much better true negative rate in the fair setting, which means that \emph{the information leakage of the fair empirical mean about the challenge point is much more than that of the empirical mean}. In addition, we also report the privacy risk, which is the maximum attack accuracy (i.e., $1- \frac{(\alpha+\beta)}{2}$) over all possible attacks. As $n_0$ decreases, the attack accuracy increases significantly in the fair setting. On the other hand, the accuracy is barely changed in the standard setting.

Besides, in the same setting (i.e., ${\sigma_0 = 1}$, ${\sigma_1 = 2}$, ${\mu_0=0}$, ${\mu_1=2}$, ${n_1=400}$), when $n_0=10$, the subgroup privacy risk in the standard setting is $50.1\%$ for both group $G_0$ and group $G_1$.
On the contrary, in the fair setting, the subgroup privacy risk is $55.1\%$ for group $G_0$ and $50.2\%$ for group $G_1$. It shows that the changes in the privacy risk caused by the fairness requirement are different for each group.


